Probing Proton Spin Structure: A Measurement of g2p at Four-momentum Transfer of 2 to 6 GeV^2

The Spin Asymmetries of the Nucleon Experiment investigated the spin structure of the proton via inclusive electron scattering at the Continuous Electron Beam Accelerator Facility at Jefferson Laboratory in Newport News, VA. A double--polarization measurement of polarized asymmetries was performed using the University of Virginia solid polarized ammonia target with target polarization aligned longitudinal and near transverse to the electron beam, allowing the extraction of the spin asymmetries $A_1$ and $A_2$, and spin structure functions $g_1$ and $g_2$. Polarized electrons of energies of 4.7 and 5.9 GeV were scattered to be viewed by a novel, non-magnetic array of detectors observing a four-momentum transfer range of 2 to 6 GeV$^2$. This document addresses the extraction of the spin asymmetries and spin structure functions, with a focus on spin structure function $g_2$, which we have measured as a function of $x$ and $W$ in four $Q^2$ bins.

==> jdm_theory.tex <==
\chapter{Nucleon Spin Structure}
\section{Overview}

\begin{equation}
 g_1(x,Q^2) = \frac{1}{2}\sum e^2_i\left[q^+_i(x,Q^2)-q^-_i(x,Q^2)\right]
\end{equation}

